Test-Time Backdoor Attacks on Multimodal Large Language Models

Backdoor attacks are commonly executed by contaminating training data, such that a trigger can activate predetermined harmful effects during the test phase. In this work, we present AnyDoor, a test-time backdoor attack against multimodal large language models (MLLMs), which involves injecting the backdoor into the textual modality using adversarial test images (sharing the same universal perturbation), without requiring access to or modification of the training data. AnyDoor employs similar techniques used in universal adversarial attacks, but distinguishes itself by its ability to decouple the timing of setup and activation of harmful effects. In our experiments, we validate the effectiveness of AnyDoor against popular MLLMs such as LLaVA-1.5, MiniGPT-4, InstructBLIP, and BLIP-2, as well as provide comprehensive ablation studies. Notably, because the backdoor is injected by a universal perturbation, AnyDoor can dynamically change its backdoor trigger prompts/harmful effects, exposing a new challenge for defending against backdoor attacks. Our project page is available at https://sail-sg.github.io/AnyDoor/.

==> Tables/demo.tex <==
\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> Tables/tab1_back.tex <==
\begin{table*}[t]
\caption{\textbf{default table}. Dataset: \textbf{VQA V2 \& SVIT \& DALLE3}; three attacks, llava-7b; trigger: SUDO, target string: I want to destroy the whole world together.}
\label{tab1:main}
\vskip 0.15in
\begin{center}
\begin{footnotesize}
% \begin{small}
\renewcommand*{\arraystretch}{1.1}
    \begin{tabular}{llccccccc}
    \toprule[1pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Attack} & \multirow{2}{*}{Sample} & \multirow{2}{*}{Budget} & \multirow{2}{*}{Size} & \multicolumn{2}{c}{\textbf{With Trigger}} & \multicolumn{2}{c}{\textbf{Without Trigger}}  \\
& & & & & ExactMatch & Contain & B@4 & ROUGE\_L \\ 
% & Batch & Epoch & Clean & AutoAttack \\
\midrule
\multirow{12}{*}{{\begin{tabular}{c}\textbf{VQAv2}
                \end{tabular}}} & \multirow{4}{*}{Pixel Attack} & 40  & $\epsilon=32/255$ & - & 52.5 & 53.5 & 34.3 & 65.4 \\
    &  & 40  & $\epsilon=48/255$ & - & 0.565 & 0.570 & 0.300 & 0.623 \\
    &  & 80  & $\epsilon=32/255$ & - & 0.575 & 0.610 & 0.364 & 0.673 \\
    &  & 80  & $\epsilon=48/255$ & - & 0.840 & 0.840 & 0.302 & 0.632 \\
\cmidrule{2-9}
& \multirow{4}{*}{Four Corner Attack} & 40  & - & $p=32$ & 0.030 & 0.030 & 0.601 & 0.802 \\
    & & 40  & - & $p=48$ & 0.875 & 0.880 & 0.449 & 0.688 \\
    & & 80  & - & $p=32$ & 0.505 & 0.510 & 0.252 & 0.594 \\
    & & 80  & - & $p=48$ & 0.875 & 0.895 & 0.463 & 0.722 \\
\cmidrule{2-9}
& \multirow{4}{*}{Border Attack} & 40  & - & $b=6$ & 0.895 & 0.895 & 0.451 & 0.731 \\
    & &  40  & - & $b=8$ & 0.870 & 0.890 & 0.333 & 0.614 \\
    & &  80  & - & $b=6$ & 0.885 & 0.885 & 0.500 & 0.767 \\
    & &  80  & - & $b=8$ & 0.920 & 0.930 & 0.416 & 0.706 \\

\midrule

\multirow{12}{*}{{\begin{tabular}{c}\textbf{SVIT}
                \end{tabular}}} & \multirow{4}{*}{Pixel Attack} & 40  & $\epsilon=32/255$ & - & 0.615 & 0.615 & 0.326 & 0.518 \\
    &  & 40  & $\epsilon=48/255$ & - & 0.775 & 0.775 & 0.309 & 0.530 \\
    &  & 80  & $\epsilon=32/255$ & - & 0.450 & 0.450 & 0.329 & 0.529 \\
    &  & 80  & $\epsilon=48/255$ & - & 0.800 & 0.800 & 0.308 & 0.528 \\
\cmidrule{2-9}                
& \multirow{4}{*}{Four Corner Attack} & 40  & - & $p=32$ & 0.650 & 0.650 & 0.337 & 0.543 \\
    & & 40  & - & $p=48$ & 0.960 & 0.960 & 0.282 & 0.498 \\
    & & 80  & - & $p=32$ & 0.885 & 0.890 & 0.370 & 0.588 \\
    & & 80  & - & $p=48$ & 0.700 & 0.700 & 0.337 & 0.561 \\
\cmidrule{2-9}
& \multirow{4}{*}{Border Attack} & 40 & - & $b=6$ & 0.950 & 0.950 & 0.414 & 0.613 \\
    & &  40  & -  & $b=8$ & 0.950 & 0.950 & 0.414 & 0.604 \\
    & &  80  & -  & $b=6$ & 0.900 & 0.900 & 0.383 & 0.585 \\
    & &  80  & -  & $b=8$ & 0.725 & 0.725 & 0.410 & 0.617 \\

\midrule

\multirow{12}{*}{{\begin{tabular}{c}\textbf{DALLE-3}
                \end{tabular}}} & \multirow{4}{*}{Pixel Attack} & 40  & $\epsilon=32/255$ & - & 0.725 & 0.725 & 0.489 & 0.764 \\
    &  & 40  & $\epsilon=48/255$ & - & 0.905 & 0.905 & 0.451 & 0.735 \\
    &  & 80  & $\epsilon=32/255$ & - & 0.865 & 0.865 & 0.486 & 0.753 \\
    &  & 80  & $\epsilon=48/255$ & - & 0.960 & 0.960 & 0.407 & 0.710 \\
\cmidrule{2-9}                
& \multirow{4}{*}{Four Corner Attack} & 40  & - & $p=32$ & 0.850 & 0.850 & 0.507 & 0.784 \\
    & & 40  & - & $p=48$ & 0.950 & 0.950 & 0.441 & 0.738 \\
    & & 80  & - & $p=32$ & 0.850 & 0.850 & 0.514 & 0.787 \\
    & & 80  & - & $p=48$ & 0.795 & 0.795 & 0.444 & 0.743 \\
\cmidrule{2-9}
& \multirow{4}{*}{Border Attack} & 40 & - & $b=6$ & 0.955 & 0.955 & 0.466 & 0.760 \\
    & &  40  & -  & $b=8$ & 0.965 & 0.965 & 0.446 & 0.742 \\
    & &  80  & -  & $b=6$ & 1.000 & 1.000 & 0.453 & 0.750 \\
    & &  80  & -  & $b=8$ & 0.885 & 0.885 & 0.503 & 0.774 \\
    

    \bottomrule[1pt]
    \end{tabular}%
\end{footnotesize}
% \end{small}
\end{center}
\vskip -0.1in
\end{table*}




% \begin{table*}[t]
% \caption{\textbf{default table}. Dataset: \textbf{VQA V2 \& SVIT \& DALLE3}; three attacks}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% % \begin{sc}
% \begin{adjustbox}{width=\textwidth}
% % \begin{adjustbox}{width=\textwidth, height=7cm}
%     \begin{tabular}{ l|l | ccccc|cc}
%     \toprule
%     % \toprule
%          % \multirow{2}{*}{MLLM} & \multirow{2}{*}{Dataset} & \multirow{2}{*}{Attack} & \multicolumn{8}{c}{Validation Set} \\
%          % \multirow{3}{*}{Dataset} & \multirow{3}{*}{Attack} & \multicolumn{8}{c}{Validation Set} \\
%          %  & & \multicolumn{5}{c|}{Without Trigger} & \multicolumn{3}{c}{With Trigger}  \\

%         \multirow{2}{*}{Dataset} & \multirow{2}{*}{Attack} & \multicolumn{5}{c|}{\textbf{Without Trigger}} & \multicolumn{2}{c}{\textbf{With Trigger}}  \\
          
%          & & B@4 & METEOR & ROUGE\_L & CIDEr & SPICE & ExactMatch & StartWith\\ 
%          \midrule
         
%           \multirow{3}{*}{VQAv2 \cite{Goyal2016MakingTV_vqav2}} & {Pixel Attack} &  1 & 1 & 1 & 1 & 1   \\
%          & {Four Corner Attack} & 
%          \\
%          & {Border Attack} &  \\
%          \midrule
         
%          \multirow{3}{*}{SVIT \cite{Zhao2023SVITSU_svit}} &  {Pixel Attack} &   \\
%          & {Four Corner Attack} & 
%          \\
%          & {Border Attack} &   \\
%          \midrule
         
%          \multirow{3}{*}{DALLE3 \cite{Ramesh2022HierarchicalTI_dalle2}} &  {Pixel Attack} &   \\
%          & {Four Corner Attack} & 
%          \\
%          & {Border Attack} &  \\
         
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% % \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}
